An RLS-Based Instantaneous Velocity Estimator for Extended Radar Tracking

Radar sensors have become an important part of the perception sensor suite due to their long range and their ability to work in adverse weather conditions. However, several shortcomings such as large amounts of noise and extreme sparsity of the point cloud result in them not being used to their full potential. In this paper, we present a novel Recursive Least Squares (RLS) based approach to estimate the instantaneous velocity of dynamic objects in real-time that is capable of handling large amounts of noise in the input data stream. We also present an end-to-end pipeline to track extended objects in real-time that uses the computed velocity estimates for data association and track initialisation. The approaches are evaluated using several real-world inspired driving scenarios that test the limits of these algorithms. It is also experimentally proven that our approaches run in real-time with frame execution time not exceeding 30 ms even in dense traffic scenarios, thus allowing for their direct implementation on autonomous vehicles.

==> resources/backup/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:experimental-setup}
All the experiments described in this section have been performed using Renault Zoes equipped with multiple Continental radars in the front and rear bumpers as shown in Figure \ref{fig:renault-zoe}.
Henceforth, the vehicle performing the tracking will be referred to as the \textit{tracker}, and the vehicle being tracked will be referred to as the \textit{trackee}. The true velocity of the trackee is obtained by using an IMU in conjunction with Wheel Speed Sensors with an accuracy of 0.1 m/s, and the true position is obtained by using a LiDAR coupled with pre-annotated High-Definition (HD) maps and GPS receivers with centimetre accuracy. 
The performance of various parts of the the algorithm is evaluated using two distinct scenarios as shown in Figure \ref{fig:expt-scenarios}. In Scenario A the tracker follows the trackee around a $\sim$\SI{750}{\meter} long test track, and in Scenario B the tracker is stationary and the trackee drives towards the tracker.

\subsection{Velocity Estimation}
\label{subsec:experiment-velocity}
In this set of experiments we evaluate the performance of our RLS-based velocity estimation algorithm. Figures \ref{fig:loop-gt-vel-comp} and \ref{fig:loop-algo-vel-comp} compare the performance of our algorithm with the estimated velocity from cluster accumulation history and ground truth from the trackee, and to other widely used algorithms like Ordinary Least Squares (OLS) and RANSAC followed by OLS for scenario A, respectively. It can be seen in Figure \ref{fig:loop-gt-vel-comp} that the RLS algorithm is able to accurately estimate the velocity of the trackee over extended periods of time. Some deviation can be observed around \SI{32}{\s} when the algorithm underestimates the velocity of trackee by around \SI{0.5}{\meter/\s} and this can be attributed to an error in ego-vehicle motion compensation causing the compensated range rate of the trackee to be lower than the true value. Additionally, some outlier values observed around \SI{52}{\s} can be attributed to measurements being included from other clusters. Because the velocity is estimated before the track-cluster association, the clusters cannot be filtered based on track IDs resulting in some values from other clusters being included in the final output. In addition, the extreme points that appear in the plot can be attributed to the few cases when the algorithm is unable to filter out all the noise points and is said to have failed. Lastly, it is worth emphasising that the velocity obtained directly from the cluster accumulation history is very noisy and cannot be directly used to estimate the velocity of a cluster, but using it as an initial seed for the RLS filter results in very accurate velocity estimates.
Furthermore, it is evident from Figure \ref{fig:loop-algo-vel-comp} that our algorithm almost always performs better than the other widely used algorithms i.e. OLS and RANSAC followed by OLS. OLS fails because of the presence of large outliers which pull the solution away from the true value, whereas RANSAC is not always able to remove all the outliers due to the dearth of points in the cluster resulting in an incorrect solution from the subsequent application of OLS.

\begin{figure}
	\centering
  \begin{subfigure}[b]{\columnwidth}
  	\centering
   	\includegraphics[width=0.9\linewidth]{images/loop_gt_comp_v3.png}
    % \setlength{\abovecaptionskip}{0pt}
    % \caption{}
    \label{fig:loop-gt-vel-comp}
  \end{subfigure}
  \begin{subfigure}[b]{\columnwidth}
    \centering
   	\includegraphics[width=0.9\linewidth]{images/loop_algo_comp_v3.png}  
    % \setlength{\abovecaptionskip}{0pt}
    % \caption{}
    \label{fig:loop-algo-vel-comp}
  \end{subfigure}
  \setlength{\abovecaptionskip}{-8pt}
  \setlength{\belowcaptionskip}{-10pt}
  \caption{Comparison of the estimated velocity between our RLS-based algorithm and that of (a) the track history and ground truth from the trackee, and (b) the velocity estimated by OLS, and RANSAC followed by OLS over a \SI{750}{\meter} long track as described by scenario A. It is evident that our algorithm is consistent with the ground truth and notably outperforms the other two algorithms.}
\end{figure}

Figure \ref{fig:straight-gt-vel-comp} compares the performance of our tracker to the initial velocity from cluster accumulation history and the ground truth from the trackee for Scenario B. It can be noted that our algorithm is able to accurately estimate the velocity of the trackee both during the acceleration and deceleration phases. The gap in the output of our algorithm from around \SI{9}{\s} to \SI{11}{\s} is because the distance between the tracker and the trackee is smaller than the minimum allowed distance from the radar resulting in it not picking up any measurements. The extreme values in the plot, like the two points measured at around \SI{7}{\s}, are due to our algorithm not being able to filter out all the outliers and can be thought of as a failure of our algorithm.
The superior performance of our algorithm is also evident in Figure \ref{fig:straight-algo-vel-comp}. OLS fails terribly because of the lack of noise handling capabilities. RANSAC followed by OLS, however, performs much better because most of the the outliers have successfully been removed by RANSAC and for this scenario we can say that this algorithm is comparable in performance to that of ours.

\begin{figure}
	\centering
  \begin{subfigure}[b]{\columnwidth}
  	\centering
   	\includegraphics[width=0.9\linewidth]{images/straight_gt_comp_v2.png}
    % \setlength{\abovecaptionskip}{0pt}
    % \caption{}
    \label{fig:straight-gt-vel-comp}
  \end{subfigure}
  \begin{subfigure}[b]{\columnwidth}
    \centering
   	\includegraphics[width=0.9\linewidth]{images/straight_algo_comp_v2.png}  
    % \setlength{\abovecaptionskip}{-10pt}
    % \setlength{\belowcaptionskip}{-5pt}
    % \caption{}
    \label{fig:straight-algo-vel-comp}
  \end{subfigure}
  \setlength{\abovecaptionskip}{-8pt}
  \setlength{\belowcaptionskip}{-10pt}
  \caption{Comparison of the estimated velocity for scenario B between our RLS-based algorithm and (a) the velocity from cluster accumulation history and the ground truth velocity from the trackee and (b) the velocity estimated by OLS, and RANSAC followed by OLS. It can be noted that our algorithm performs well as compared to the ground truth and is significantly better than OLS. RANSAC followed by OLS is able to discard the a lot of noise points and its performance in this scenario is comparable to that of ours.}
\end{figure}

\subsection{Tracking Performance}
\label{subsec:experiment-tracking-performance}
In this section we evaluate the tracking performance of the our extended object tracker using two metrics, namely, the positional tracking accuracy and the object dimension tracking accuracy using scenario A. Figure \ref{fig:loop-gt-trk-comp} depicts the position of the tracked object as computed by the tracker as compared to the ground truth position of the trackee. It can be noted that the tracker is very accurate along the straights but overestimates the radius and deviates from the ground truth during turns. This deviation can be attributed to the requirement of having a smooth track resulting in the Kalman Filter tuning giving more weight to the prediction than to the new measurements. Because the velocity vector is tangential to curve, the prediction step pushes the predicted position out of the circle. The measurement update then partially pulls the position towards the circle resulting in overestimation of the radius during turns.
On the other hand, the deviations of the tracker on the straights like the ones observed at coordinates $(45, -15)$ and $(-65, -45)$ are due to several erroneous points appearing on the road surface. Because of the proximity of these measurements to the true ones, they are clustered together resulting in incorrect measurement update of the Kalman Filter and subsequently an incorrect track position.

Figure \ref{fig:loop-gt-extents-comp} compares the estimation of the dimensions of the trackee with that of the ground truth. As stated in \ref{subsubsec:cluster-no-track} the length and width are initialised to \SI{4}{\meter} and \SI{2}{\meter} respectively when the track is first created and they are then constantly updated as part of the measurement update step of the Kalman Filter. The initial sharp drop can be explained by the lack of measurements with range rate greater than the pre-defined threshold on the trackee resulting in the length and width being severely underestimated. Once the cars start moving more points pass through the filter which immediately improves the dimension estimates. Additionally, it can be seen that the width is always under-estimated by the tracker and this can be attributed to the relatively large angular resolution of the radar which limits the number of points width-wise resulting in such a behaviour.

% to the radar waves reflecting off water puddles on the road surface resulting in

\begin{figure}
	\centering
  \begin{subfigure}[b]{\columnwidth}
  	\centering
   	\includegraphics[width=0.6\linewidth]{images/loop_tracker_pos_gt_comp_v1.png}
    % \setlength{\abovecaptionskip}{2pt}
    % \caption{}
    \label{fig:loop-gt-trk-comp}
  \end{subfigure}
  \begin{subfigure}[b]{\columnwidth}
    \centering
   	\includegraphics[width=0.9\linewidth]{images/loop_extents_v2.png}  
    % \setlength{\abovecaptionskip}{-10pt}
    % \setlength{\belowcaptionskip}{-5pt}
    % \caption{}
    \label{fig:loop-gt-extents-comp}
  \end{subfigure}
  \setlength{\abovecaptionskip}{-8pt}
  \setlength{\belowcaptionskip}{-15pt}
  \caption{Evaluation of the tracking performance using two metrics, namely, position and extents. Plot (a) overlays the ground truth position of trackee over the tracked estimates from the tracker. Very few deviations from the true path are observed, thus proving the positional accuracy of our tracker. Plot (b) compares the estimated extents with the ground truth from which we can infer that although the length estimate is quite accurate, the width of the trackee is always underestimated by the tracker due to the dearth of points in the width-wise direction.}
\end{figure}

\subsection{Runtime}
\label{subsec:experiment-runtime}
Figure \ref{fig:one-north-runtime} plots the runtime of both the overall extended tracking pipeline right from the clustering phase till the end of the pipeline and the RLS-based velocity estimation module in real-world traffic with the number of objects ranging from 5 to 30 objects per frame. It can be seen that the algorithm runs in real time with the RLS module taking around \SI{0.89}{\milli\s} on average for all the clusters in a frame. Similarly, the entire tracker also runs in real time using around \SI{2.1}{\milli\s} per frame on average. We can thus safely say that our extended object tracking algorithm can run in real time even in dense traffic scenarios. 

\begin{figure}
	\centering
  \begin{subfigure}[b]{\columnwidth}
  	\centering
   	\includegraphics[width=\linewidth]{images/dense_traffic.png}
    % \setlength{\abovecaptionskip}{2pt}
    % \caption{}
    \label{fig:dense-traffic-image}
  \end{subfigure}
  \begin{subfigure}[b]{\columnwidth}
  	\centering
   	\includegraphics[width=0.9\linewidth]{images/one_north_runtime_v2.png}
    % \setlength{\abovecaptionskip}{2pt}
    % \caption{}
    \label{fig:one-north-runtime}
  \end{subfigure}
  \setlength{\abovecaptionskip}{-8pt}
  \setlength{\belowcaptionskip}{-15pt}
  \caption{(a) A frame of the dense traffic as seen by the front cameras containing 15 objects of interest. (b) Runtime of both the overall extended object tracking pipeline and the RLS-based instantaneous velocity estimation module. It is worth noting that both the RLS algorithm and the overall pipeline run in real time, thus allowing its implementation on autonomous vehicles.}
\end{figure}


==> resources/backup/problem-statement.tex <==
\section{Problem Statement}
\label{sec:problem-statement}
The objective of this work is to enable the accurate estimation of instantaneous velocity of dynamic objects in real-time using measurements from only the Radar sensors. 
To ensure the applicability of our approach to a wide range of objects, only the raw measurements from the Radar sensor like the range rate and azimuthal angle are used and no model assumptions are made.
Two main challenges faced when working with only the Radar sensor are (i) the sparsity of input data and (ii) large amounts of sensor noise especially in the range rate measurements. 


